Flextron: Many-in-One Flexible Large Language Model

Training modern LLMs is extremely resource intensive, and customizing them for various deployment scenarios characterized by limited compute and memory resources through repeated training is impractical. In this paper, we introduce Flextron, a network architecture and post-training model optimization framework supporting flexible model deployment. The Flextron architecture utilizes a nested elastic structure to rapidly adapt to specific user-defined latency and accuracy targets during inference with no additional fine-tuning required. It is also input-adaptive, and can automatically route tokens through its sub-networks for improved performance and efficiency. We present a sample-efficient training method and associated routing algorithms for systematically transforming an existing trained LLM into a Flextron model. We evaluate Flextron on the GPT-3 and LLama-2 family of LLMs, and demonstrate superior performance over multiple end-to-end trained variants and other state-of-the-art elastic networks, all with a single pretraining run that consumes a mere 7.63% tokens compared to original pretraining.

==> tex/background.tex <==
\section{Background}

In this section, we first formally define a generalizable framwork for elastic inference (Sec~\ref{sec:background:framework}), and show that existing works are its special case (Sec~\ref{sec:background:existing}).

\subsection{Generalizable Framework for Elastic Inference} \label{sec:background:framework}

Given a model $\mathcal{M}$ of $N$ layers, each layer could be formalized as $\boldsymbol{y} = l^{i}(\boldsymbol{x}, W^{i})$, where $i$ refers to the layer index and $W^{i}$ denotes the parameters of the layer. For a static model, during inference, the $W^{i}$ should remain untouched for the model efficacy, leading to the fixed memory usage and latency. For flexibility of model deployment, we extend the static weight matrix to a elastic form, formally, 
\begin{equation}
    W^{i}_e = g(W^{i}, h, \boldsymbol{x}),
\end{equation}
where $g$ refers to the generation function, which takes the original weight $W^{i}$, hardware requirement $h$, and data $\boldsymbol{x}$ as input, and output the $W^{i}_e$. By replacing $W^{i}$ with $W^{i}_e$, the model could be transformed into a more compact form, enabling the flexible deployment.

\subsection{Existing Works} \label{sec:background:existing}


